On Phase Offsets of 802.11ac Commodity WiFi

We analyze the phase offsets between RF chains of modern IEEE 802.11ac chips. We investigate both the 2.4 and 5GHz bands on a per OFDM subcarrier level. Results reveal that the phase offset between receive antennas is due to random phase rotations semi-time-invariant with up to four possible values. Moreover, it is frequency-dependent. We propose a simple algorithm, which allows us to correct the phase offset on the fly without any calibration. As proof-of-concept, we implemented Angle of Arrival (AoA) using MUSIC algorithm. To achieve higher accuracy we stitched the thirteen overlapping 20MHz channels available in 2.4GHz band together to effectively have a single 80MHz channel. Results show very good AoA precision although only two receive antennas were used.

==> sections/primer.tex <==
%!TEX root = ../main.tex

%%%
\section{CSI Primer}
%
RF signals like WiFi can be used beyond transmission of data. 
%
This is because the RF signal generated by the transmitter propagates through multiple paths, such as direct propagation (radiation), reflection and scattering, and superimposes at the receiver, carrying the information of the characteristics of the propagated environment, the so-called Channel State Information (CSI). 
%
The best known application is the radar system used to localize airplanes.
%
%\tolja{TBD: need more meat here.}
